Many-to-many Image Generation with Auto-regressive Diffusion Models

Recent advancements in image generation have made significant progress, yet existing models present limitations in perceiving and generating an arbitrary number of interrelated images within a broad context. This limitation becomes increasingly critical as the demand for multi-image scenarios, such as multi-view images and visual narratives, grows with the expansion of multimedia platforms. This paper introduces a domain-general framework for many-to-many image generation, capable of producing interrelated image series from a given set of images, offering a scalable solution that obviates the need for task-specific solutions across different multi-image scenarios. To facilitate this, we present MIS, a novel large-scale multi-image dataset, containing 12M synthetic multi-image samples, each with 25 interconnected images. Utilizing Stable Diffusion with varied latent noises, our method produces a set of interconnected images from a single caption. Leveraging MIS, we learn M2M, an autoregressive model for many-to-many generation, where each image is modeled within a diffusion framework. Throughout training on the synthetic MIS, the model excels in capturing style and content from preceding images - synthetic or real - and generates novel images following the captured patterns. Furthermore, through task-specific fine-tuning, our model demonstrates its adaptability to various multi-image generation tasks, including Novel View Synthesis and Visual Procedure Generation.

==> figures/content_consistency.tex <==
\begin{figure}[!t]
    \centering
\includegraphics[width=\linewidth]{figures/content.pdf}
    \caption{\textbf{Content Consistency.} Top panel for \shortsdmodel{}, bottom for \shortdinomodel{}, both featuring three rows. In each row, Columns 1-4 display preceding images, and Columns 5-8 are the generated images.}
    \label{fig:content_consis}
\end{figure}



==> figures/dino_score.tex <==
\begin{figure}[!t]
    \centering
\includegraphics[width=\columnwidth]{}
    \caption{\textbf{Evaluation Metrics for Image Generation by \shortdinomodel{}} FID (\downarrow) (a), IS (\uparrow) (b), Text-Image CLIP (\uparrow) (c), and Image-Image CLIP (\uparrow) (d) of images generated conditioned on four preceding images. The horizontal axis is the number of generated images and the vertical axis shows the different evaluation metrics. 
    The blue line charts the score for each generated image, while the dashed orange line marks the average score across all generated images.}
    \label{fig:dino_score}
\end{figure}



==> figures/image_set_attn_fig.tex <==
\begin{figure}[!t]
    \centering
\includegraphics[width=\columnwidth]{figures/image_set_attn.pdf}
    \caption{\textbf{Illustration of \multiimageattn{} Module.} This figure demonstrates the two core components of the \multiimageattn{} module (Block-size $B$ = 2): (a) the \globalattn{} module and (b) the \blocksetattn{} module. The query token is denoted in a white square and its corresponding key/value attention region is marked by a diagonal striped pattern.}
    \label{fig:image_set_attn}
\end{figure}



==> figures/style_consistency.tex <==
\begin{figure*}[!t]
    \centering
\includegraphics[width=\linewidth]{figures/style.pdf}
    \caption{\textbf{Style Consistency.} }
    \label{fig:style_consis}
\end{figure*}

==> sections/3_method_mix.tex <==
\input{figures/overview_fig}

\section{\longmodelname{} (\shortmodelname{})}
\label{sec:method}


We introduce the \longmodelname{} (\shortmodelname{}) framework, designed to perceive and generate an arbitrary number of interrelated images auto-regressively, as illustrated in Figure \ref{fig:overview}. 
% This model is adept at producing new images that maintain a semantic relationship with a given sequence of preceding images.
% For any given an arbitrary number of interrelated preceding images $I^{1:K}$, our proposed model generates an arbitrary number of novel images that have interconnected with the preceding images in an auto-regressive manner.
Our framework extends the pre-trained Stable Diffusion, the large-scale text-to-image latent diffusion model. Central to Stable Diffusion is the denoising model $\epsilon_{\theta}(\cdot)$, which is built upon the U-Net, but further enriched with a text-to-image cross-attention layer. 
We modify the architecture by supplanting the text-to-image cross-attention module with our Image-Set Attention module, which allows the model to learn and understand the intricate interconnections within a set of images, thereby facilitating more contextually coherent multi-image generation.

Our framework explores different architectural approaches for multi-image generation. The key differentiator among these approaches lies in their methods for encoding and applying attention to preceding images.
In Section \ref{sec:blockmix}, we introduce \textbf{\blockmix{} (\shortblockmix{})}, utilizing the U-Net-based denoising model  $\epsilon_{\theta}(\cdot)$ for simultaneously processing the preceding latent images and the noisy latent images. This allows for a more sophisticated cross-attention over the preceding images, facilitating the generation of new images that are contextually and semantically linked to the preceding images.
Additionally, Section \ref{sec:dinomodel} details \textbf{\dinomodel{} (\shortdinomodel{})}, which investigates the incorporation of external vision models for encoding the preceding images, aiming to complement the U-Net's inherent capabilities for encoding the preceding images

% \blockmix{} and \dinomodel{}
% Within the \multiimageattn{} module, we aim to facilitate cross-attention from noisy latent images to preceding clean latent images.

\section{\blockmix{} (\shortblockmix{})}
\label{sec:blockmix}

During the training phase, given an image set $\{I\}_{i=1}^N$, each image $I_i$ is first encoded individually into the latent code $z_0^i$ using a pre-trained autoencoder $z_0^i = \mathcal{E}(I_i)$. These image latents are then stacked to construct $z_0^{1:N} \in \mathbb{R}^{N \times C \times H \times W}$, where $N$ represents the number of images within each set, $C$ is the number of latent channels, and $H$ and $W$ are the spatial dimensions of the latent space.
The latent $z_0^{1:N}$ is subsequently noised according to the pre-defined forward diffusion schedule to produce the noisy latent $z_t^{1:N}$, where the noise level increases over diffusion timesteps $t$. 

To prepare the input for \blockmix{}, we concatenate the noisy and clean latent codes, resulting in $z^{1:N} = [z_0^{1:N}; z_t^{1:N}] \in \mathbb{R}^{2 \times N \times C \times H \times W}$. Here, the symbol $;$ denotes the concatenation operation and the factor $2$ reflects the inclusion of both clean and noised latent forms.
Our model takes the combination of clean latent images and their corresponding noisy latent images as inputs and then predicts the noise added to the noised latent images in an auto-regressive manner.

\subsection{\multiimageattn{}}

The core component in \blockmix{} is the \multiimageattn{} module, designed effectively facilitate cross-attention from noisy latent images to preceding clean latent images.

The \multiimageattn{} module accepts an input tensor $z \in \mathbb{R}^{BZ \times 2 \times N \times H \times W \times C}$, where $BZ$ stands for batch size. For readability, the superscript $1:N$ has been omitted. The input $z$ is first partitioned and reshaped into the following two components: the noisy latent $z_n \in \mathbb{R}^{BZ \times N \times H \times W \times C}$ and its corresponding clean latent $z_c \in\mathbb{R}^{BZ \times N \times H \times W \times C}$. 
\multiimageattn{} implements a blockwise attention strategy by partitioning the image set into smaller blocks. In particular, the image dimension $N = K * B$ is segmented into $K$ blocks, each containing $B$ images. This results in a reshaped structure of both noisy and clean latent as $BZ \times K \times B \times H \times W \times C$.

The attention mechanism within \multiimageattn{} operates in two-stages, starting with \textbf{\blockselfattn{}} mechanisms within individual image blocks to capture contextual details and then \textbf{\blockcrossattn{}} across noisy and clean image blocks.

\subsubsection{\blockselfattn{}}

\blockselfattn{} operates within each noisy image block, capturing intra-block contextual information. The self-attention follows the scaled dot-product attention layer introduced by \cite{vaswani2017attention}, represented mathematically as:

\begin{align}
    z'_n = \text{Attention}(Q, K, V) = \text{Softmax}(\frac{QK^T}{\sqrt{d}}) \cdot V,
\label{eq:attn}
\end{align}
where $Q = W^Q z^Q$, $K = W^K z^K$, and $V = W^V z^V$ denotes the three projections of the reshaped latents and $d$ is the dimension of the latent feature.
The self-attention operates with the noised latents as queries, keys and values $z^Q = z^K = z^V = z_n \in \mathbb{R}^{(BZ \times K) \times (B \times H \times W) \times C}$. We also make the attention multi-head, allowing the model to jointly attend to information from different representation subspace~\cite{vaswani2017attention}.

 As illustrated in Figure \ref{fig:image_set_attn} (a), for each noisy patch that acts as the queries and belongs to the $k$-th block of noisy latents, all the noisy patches from the same $k$-th block are served as keys and values.

\subsubsection{\blockcrossattn{}}

The \blockcrossattn{} module, as illustrated in Figure \ref{fig:image_set_attn} encompasses two distinct cross-attention attention mechanisms: (b1) \textbf{\globalattn{}} and (b2) \textbf{\blocksetattn{}}. 
Considering the inherent structure of the U-Net architecture, which includes a series of contraction and expansion blocks operating at varying spatial dimensions, \blockcrossattn{} proposes to employ \globalattn{} in blocks with small spatial dimensions, and \blocksetattn{} in blocks with large spatial dimensions. \globalattn{} is designed to attend to all patches of preceding image blocks, providing a comprehensive cross-attention scope. Conversely, \blocksetattn{} applies cross-attention along the set axis, attending only to patches in the preceding image blocks at the same spatial location. 

\paragraph{\globalattn{}}

Recall that, the noisy and clean latents initially shaped as $BZ \times K \times B \times H \times W \times C$. \globalattn{}, are reshaped into $z_n \in \mathbb{R}^{BZ \times (K \times B \times H \times W) \times C}$. This transformation facilitates a comprehensive attention across the resultant length of $K \times B \times H \times W$. 

In the context of \globalattn{}, the scaled dot-product cross-attention layer, as per Equation \ref{eq:attn}, is employed where the noised latents serve as queries $z^Q = z_n$ and the clean latents function as keys and values $z^K = z^V = z_c$. 
To maintain the flow of information from previous clean image blocks, a causal image-set attention mask is introduced, permitting each noisy latent $z^{b_i}_{n}$ within image block $b$ to exclusively attend to patches within its preceding clean blocks $z^{<b}_c$. 
Figure \ref{fig:image_set_attn} (b1) provides a visualization of this process, depicting an example of a query token and the key/value region it allows to attend.

Finally, \globalattn{} construct the output latent $z'$ by concatenating the original clean latent and the updated noisy latent, producing the output $z' = [z_c; z'_n] $.

\paragraph{\blocksetattn{}}

\input{figures/image_set_attn_fig}

While \globalattn{} has the benefit of allowing comprehensive interaction with all clean patches of preceding images, it also increases the computation costs in terms of memory and training time. To improve efficiency, we propose to employ \globalattn{} in U-Net blocks with small spatial dimensions. For blocks with large spatial dimensions, we consider \blocksetattn{} which performs attention along the image-set axis. Unlike, \globalattn{}, \blocksetattn{} only attends to the spatially correspondent clean patches in preceding image blocks. 
% For instance, a set of four images, when divided with a block size of two, results in two separate image blocks. This enables us to perform blockwise inference during test time.

% In the \blocksetattn{} module, both noisy and clean latent are reshaped first by segmenting the image dimension into $K$ blocks, with each block comprising $B$ images, resulting in a shape of $BZ \times K \times B \times H \times W \times C$.

The facilitate attention along the set-axis, \blocksetattn{} reshapes the clean and noisy latent into the shape of $(BZ \times H \times W) \times N \times C$. In accordance with Equation \ref{eq:attn}, the projections of the reshaped noisy latent serve as the queries, and those of the reshaped clean latent act as keys and values. We incorporate a blockwise causal attention mask, ensuring that each noisy patch exclusively attends to the patch at the same spatial location from preceding clean image blocks. Figure \ref{fig:image_set_attn} (b2) illustrates this attention mechanism between noisy and clean image latents along the image-set axis.

\section{\dinomodel{} (\shortdinomodel{})}
\label{sec:dinomodel}
% \subsection{Encoding Strategies for Preceding Images \ying{tentative}}

So far, \blockmix{} relies on the same U-Net-based denoising model for processing the preceding images as internal features. Additionally, we explores the potential advantage of integrating external vision models to encode the preceding images into discriminative visual features. Specifically, we employ the DINOv2~\cite{oquab2023dinov2} for the encoding of preceding images. The DINOv2  model pretrains the image encoder on large curated image data, which shows a superior understanding of fine-grained vision information.

In \shortdinomodel{}, each image $I_i$ from an image set $\{I\}_{i=1}^N$ is encoded individually into two distinct formats: the latent code $z_0^i$ using a pre-trained autoencoder $z_0^i = \mathcal{E}(I_i)$ and DINO features $v^i = \mathcal{E}_v(I_i)$. 
These encoded forms are then stacked to construct two forms of encoded features: $z_0^{1:N} \in \mathbb{R}^{N \times C \times H \times W}$ and $v^{1:N} \in \mathbb{R}^{N \times S \times D}$, where $N$ represents the number of images within each set, $S$ denotes the length of DINO image tokens, $D$ is the dimensionality of the DINO features.

Following the encoding process, the U-Net-based denoising model takes in the noised latent $z_t^{1:N}$, derived from $z_0^{1:N}$ through the predefined noise addition schedule.
The DINO features $v$, on the other hand, are utilized within the intermediate layers of U-Net via the Image-Set Attention module following the Equation \ref{eq:attn}. Here, the DINO features $v$ act as keys and values $z^K = z^V = v$, while the queries $z^Q$ are the noisy image latents $z_t \in \mathbb{R}^{BZ \times (N \times H \times W) \times C}$. For clarity, the superscript $1:N$ is omitted in this context. In \multiimageattn{}, \dinomodel{} only employs the \globalattn{} with a block-size=1.
 % the noisy image latents $z_t$ attends to all DINO features $v$ with a block-size=1.


\section{Training and Inference Procedure}

\subsection{Training}
\paragraph{Training Objective} The training process is similar to the Latent Diffusion Model \cite{rombach2022high}. During training, we initialize the model weights from the Stable Diffusion Model, but intentionally exclude the pre-trained text-to-image cross-attention layer. 

% Our \modelname{} takes the concatenated clean and noisy latent codes of the image sets as input and predicts the noise strength added to each noised latent image conditioned on the previous clean image latent. The auto-regressive training loss is accumulated on the predicted noise of each image, as follows:
\modelname{} takes the visual features of the clean images, denoted as $z_0^{1:N}$, and the noisy latent images, $z_t^{1:N}$, as inputs. The model's objective is to predict the noise strength added to each noised latent image conditioned on the previous clean image features. The auto-regressive training loss is accumulated on the predicted noise of each image, as follows:

% \begin{align}
%     \mathcal{L}_{\theta} = \mathbb{E}_{\mathcal{E}(x_0^{1:N}), \epsilon, t} \big{[} \| \epsilon - \epsilon_{\theta}([z_0^{1:N}; z_t^{1:N}], t) \|^2_2 \big{]}
% \end{align}

\begin{align}
    \mathcal{L}_{\theta} = \mathbb{E}_{\mathcal{E}(x_0^{1:N}), \epsilon, t} \big{[} \| \epsilon - \epsilon_{\theta}(z_t^{1:N}, z_0^{1:N}, t) \|^2_2 \big{]},
\end{align}
where $z_0^{1:N}$ is the clean image latents in \blockmix{} and $z_0^{1:N} = v^{1:N}$ is the DINO features in \dinomodel{}.
To incorporate classifier-free guidance~\cite{ho2021classifier} during sampling, the \modelname{} is jointly trained with conditional and unconditional objectives, and the conditional and unconditional score estimates are combined at inference time. Training for unconditional denoising is achieved by randomly zeroing out the clean image condition $z_0^{1:N}$ with 10\% probability.

\subsection{Inference}

As shown in Figure \ref{fig:overview}, during inference, \modelname{} can generate an arbitrary number of images in an auto-regressive manner. This is achieved by iteratively incorporating the images generated in the previous iteration as new inputs for subsequent iterations. This process begins by generating an initial image (or a block of images), utilizing a set of conditional input images and randomly sampled noise latent codes. Afterward, the model incorporates the previously generated image (or block of images) into the input context for the next generation cycle. In practice, the number of context images that can be input into the model is bounded by a predefined parameter, the context window $W$.
Note that, in \dinomodel{}, the model generates a single image in an iterative cycle, whereas \blockmix{} generates a block of images in a single iteration.

At inference time, with a guidance scale $s \geq 1$, the output of the model is extrapolated further in the direction of the conditional $\epsilon_{\theta}(z_t, z_0^{1:W}, t)$ and away from the unconditional $\epsilon_{\theta}(z_t, \mathbf{0}, t)$:

\begin{align}
    \tilde{\epsilon}_{\theta}(z_t, z_0^{1:W}, t) &= \epsilon_{\theta}(z_t, \mathbf{0}, t) \notag \\
    &\quad + s \cdot (\epsilon_{\theta}(z_t, z_0^{1:W}, t) - \epsilon_{\theta}(z_t, \mathbf{0}, t))
\end{align}

Here, $z_0^{1:W}$ represents the sequence of context images serving as the conditional inputs for the generative process.




==> tables/sampling_speed.tex <==
\begin{table}[!t]
  \centering
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{l | c c c c}
  \toprule
   \textbf{Method} & Num. of Input Images  & Num. of Generated Images  & Time per Generated Image (s) \\
  \midrule
    SD-2.1-base & - & 1 & 8 \\
    \midrule
  \shortdinomodel{} & 1 & 1  \\
  \shortdinomodel{} & 1 & 4  \\
  \shortdinomodel{} & 4 & 4  \\
  \midrule
  \shortsdmodel{}  & 1 & 1  \\
  \shortsdmodel{}  & 1 & 4  \\
  \shortsdmodel{}  & 4 & 4  \\
  \bottomrule
  \end{tabular}}
  \caption{\textbf{Sampling Efficiency.} Sampling using the DDIM sampler with 50 denoising steps on a single A40 GPU. The sampling seed is measured as the average time to generate one image.
  }
  \label{table:sampling_speed}
  \end{table}
